Revisiting the memoryless property -- testing for the Pareto type I distribution

We propose new goodness-of-fit tests for the Pareto type I distribution. These tests are based on a multiplicative version of the memoryless property which characterises this distribution. We present the results of a Monte Carlo power study demonstrating that the proposed tests are powerful compared to existing tests. As a result of independent interest, we demonstrate that tests specifically developed for the Pareto type I distribution substantially outperform tests for exponentiality applied to log-transformed data (since Pareto type I distributed values can be transformed to exponentiality via a simple log-transformation). Specifically, the newly proposed tests based on the multiplicative memoryless property of the Pareto distribution substantially outperform a test based on the memoryless property of the exponential distribution. The practical use of tests is illustrated by testing the hypothesis that two sets of observed golfers' earnings (those of the PGA and LIV tours) are realised from Pareto distributions.

==> toets.tex <==
Let $Y$ be a random variable denoting an exponential waiting time. The memoryless property of the exponential distribution can be expressed as
\begin{equation}
    P(Y \ge s+t|Y>s)=P(Y>t), \quad t,s\ge 0. \label{a}
\end{equation}

If $Y$ is exponential with mean $1/\beta$, then $X=\textrm{e}^Y$ is a Pareto distributed random variable with shape parameter $\beta>0$.

The Pareto distribution exhibits a multiplicative version of the memoryless property, which can be expressed as follows. $X \sim P(\beta)$ for some $\beta>0$ if, and only if,
\begin{equation}
     P(X \ge st|X>s)=P(X>t), \quad t,s\ge 1.\label{b}
\end{equation} 


